Inferring System and Optimal Control Parameters of Closed-Loop Systems from Partial Observations

We consider the joint problem of system identification and inverse optimal control for discrete-time stochastic Linear Quadratic Regulators. We analyze finite and infinite time horizons in a partially observed setting, where the state is observed noisily. To recover closed-loop system parameters, we develop inference methods based on probabilistic state-space model (SSM) techniques. First, we show that the system parameters exhibit non-identifiability in the infinite-horizon from closed-loop measurements, and we provide exact and numerical methods to disentangle the parameters. Second, to improve parameter identifiability, we show that we can further enhance recovery by either (1) incorporating additional partial measurements of the control signals or (2) moving to the finite-horizon setting. We further illustrate the performance of our methodology through numerical examples.

==> cdc_input.tex <==
\NeedsTeXFormat{LaTeX2e}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Structure file
% Author: Victor Geadah
% Date: 30/11/2021
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% =============================================
%   General packages
% =============================================

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

% Packages
\usepackage{amsmath, amsfonts, amssymb, amsthm} %maths 
\usepackage{soul} % for underline
% \usepackage{titling} % to call title, author, etc

% =============================================
%   Links
% =============================================

\usepackage{hyperref}
\usepackage{xcolor}

% Set link colours
\definecolor{newcolor}{rgb}{0,0.2,0.6}
\hypersetup{
    colorlinks = true,
    urlcolor = newcolor,
    linkcolor = black,
    citecolor=newcolor
}


% =============================================
%   Shortcuts & Macros
% =============================================

\newcommand{\N}{\mathbb{N}} % natural numbers
\newcommand{\Z}{\mathbb{Z}} % integers
\newcommand{\Q}{\mathbb{Q}} % rational numbers
\newcommand{\R}{\mathbb{R}} % real numbers
\newcommand{\C}{\mathbb{C}} % complex numbers
\newcommand{\E}{\mathbb{E}} % complex numbers

\newcommand{\s}[1]{\mathcal{#1}} % 'script'
\newcommand{\pdv}[1]{\frac{\partial}{\partial #1}}
\newcommand{\norm}[2][]{\left|\left|#2\right|\right|_{#1}} 
    % \norm[#2]{#1} returns || #1 ||_#2
\newcommand{\abs}[1]{\left|#1\right|}
    % \abs{#1} returns | #1 |

% =============================================
%   Theorems, etc
% =============================================

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}
%
\theoremstyle{definition}%
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}[section]

% Option-independent thm environements
\theoremstyle{remark}
\newtheorem*{remark}{Remark}


% ============================================
% Figures

\usepackage{graphicx, wrapfig}

% Tikz
\usepackage{tikz}
\usetikzlibrary{bayesnet}
\usetikzlibrary{calc}
% \usetikzlibrary{shapes.geometric, arrows}
\tikzstyle{barrow} = [->, >={triangle 45}, draw=blue]
\tikzstyle{cconst} = [circle, inner sep=0pt, node distance=1, draw=white]

